Fully Dynamic Matching: Beating 2-Approximation in $\Delta^\epsilon$ Update Time

In fully dynamic graphs, we know how to maintain a 2-approximation of maximum matching extremely fast, that is, in polylogarithmic update time or better. In a sharp contrast and despite extensive studies, all known algorithms that maintain a $2-\Omega(1)$ approximate matching are much slower. Understanding this gap and, in particular, determining the best possible update time for algorithms providing a better-than-2 approximate matching is a major open question. In this paper, we show that for any constant $\epsilon > 0$, there is a randomized algorithm that with high probability maintains a $2-\Omega(1)$ approximate maximum matching of a fully-dynamic general graph in worst-case update time $O(\Delta^{\epsilon}+\text{polylog } n)$, where $\Delta$ is the maximum degree. Previously, the fastest fully dynamic matching algorithm providing a better-than-2 approximation had $O(m^{1/4})$ update-time [Bernstein and Stein, SODA 2016]. A faster algorithm with update-time $O(n^\epsilon)$ was known, but worked only for maintaining the size (and not the edges) of the matching in bipartite graphs [Bhattacharya, Henzinger, and Nanongkai, STOC 2016].

==> tmp.tex <==
\section{Temporary Stuff}

\begin{proof}
	
	
	Consider the following equivalent way of constructing matching $M_G := \lfmm{G[W \cup U], \pi}$ that gradually reveals the subsample $W$ of $V$. 
	
	
	
	
	In the initialization step, every vertex in $G$ is marked as {\em alive} and matching $M_G$ is initialized to be $\emptyset$. If a vertex is not alive, we say it is {\em dead} and if at least one vertex of an edge is dead, we say the edge is dead. The process iterates over the edges of $G$ in the order of $\pi$. Upon visiting an edge $uv$ with $v \in V$, if $uv$ is dead, we discard it. Otherwise, we query whether $v \in W$ (this may have already been revealed during previous iterations). If $v \in W$, we add $uv$ to $M_G$ and mark both $u$ and $v$ as dead.
	
	Let us use ``time $i$'' to refer to the first moment in the process above that the size of $M_G$ becomes $i$. Define	$K(i) := \{uv \mid uv \in M, v \in W \text{ and $uv$ is dead at time $i$}\}$. Note that while at time $i$, we cannot determine the set $K(i)$ as we have not fully revealed the subsample $W$. However, we can determine the value of the following potential function that measures the \underline{expected} size of $K(i)$, where the expectation is taken over the parts of $W$ not revealed yet:
	$$
	\phi(i) = \E[|K(i)| \mid \text{randomizations revealed by time $i$}].
	$$
	We show that the conditions of Wald's equation hold for $\phi(i)$. First, observe that initially all the vertices in the graph are alive and thus $K(0) = \emptyset$ and $\phi(0) = 0$. Next, we show that for every $i$,
	\begin{equation}
	\E[\phi(i)-\phi(i-1) | \phi(i-1)] \leq 1 + p.
	\end{equation}
	We say an edge $e$ is killed at time $i$ if $e \in K(i)$ and $e \not\in K(i-1)$. With this definition,  $\phi(i)-\phi(i-1)$ would denote the expected number of edges that are killed at time $i$. Observe that during the time $i-1$ and $i$, we may have processed a set of edges, but all were discarded except the last edge $uv$ which was added to $M_G$.	This means that in this timeframe, only vertex $v$ has been revealed to be in $W$ since in the process, anytime that we query whether a vertex is in $W$ and the answer is positive, we add one edge to $M_G$. Those vertices queried between time $i-1$ and $i$ that have been identified to not be in $W$, can only decrease the expected value of $K(i)$. On the other hand, the last edge $uv$ that is added to $M_G$, can be adjacent to at most two edges in $M$ and thus can kill at most two edges of $M$.
	
	
	\vspace{2cm}
	Partition the vertices in $V$ into two subsets $\vm := V \cap V(M)$ and $\vnotm = V \setminus V_M$. Subset $\vm$ includes all vertices in $V$ that are matched in $M$ and $\vnotm$ includes the rest of the vertices in $V$. Observe that the only source of randomization in the lemma is the subsample $W$ of $V$. For the proof, we will need to be careful about the order in which we reveal which vertices in $V$ are sampled.
	
	
	
	First, for each vertex $v \in \vnotm$, we reveal whether $v \in W$ and use $\vnotmsampled := \vnotm \cap W$ to denote the set of vertices in $\vnotm$ that are sampled.
	
	Next, we construct matching $\lfmm{G[V' \cup U], \pi}$ in the following way while gradually revealing the subsampled vertices of $\vm$ only when it is needed. We iterate over the edges in the order of $\pi$.
	
	\begin{enumerate}
		\item Upon visiting an edge $uv$, it could be the case that we already know whether the bottom vertex is sampled or not. Regardless, even if it  is not, we just reveal that and this tells us whether $uv$ gets added to the greedy matching or not. 
		\item We would like to know whether another edge of $M$ whose bottom vertex is in $W$ is also killed or not. For this, we look at the top vertex of this edge $uv$. If we already have revealed whether its bottom vertex is sampled, and it is indeed sampled, then another vertex has already killed it. Therefore, we don't know this and it happens with probability $p$.
		\item Each step, kills at most $1+p$ edges of $M \cap V'$. Thus, it takes by wald's equation, $p|M|/(1+p)$ steps to kill them all. Each step is an edge in the matching, thus the matching size is at least this much.
		\item Now, we care only about those edges of the matching that have their endpoint in $\vm$. If there are $Y$ vertices sampled in $\vnotm$, then clearly we have 
	\end{enumerate}
\end{proof}

\begin{tboxalg2e}{}
	\begin{algorithm}[H]
		\DontPrintSemicolon
		\SetAlgoSkip{bigskip}
		\SetAlgoInsideSkip{}
		
		Mark every vertex in $G$ as {\em alive}. If a vertex is not alive we say it is {\em dead.} If at least one endpoint of an edge is dead, we say the edge is dead.\;
		Initialize $M_G \gets \emptyset$.\tcp*{This will be equivalent to matching \lfmm{G[W \cup U],\pi} in the end.}
		$\phi \gets 0$. \tcp*{Invariant: $\phi$ will be the number of dead edges $uv \in M$ where $v \in W$.}
		\For{edge $uv \in E$ with $v \in V$ (the edges are iterated over in this for-loop in the order of $\pi$)}{
			\If{at least one of $u$ or $v$ is dead}{
				Discard $uv$.	
			}\Else{
				If not revealed so far, reveal whether $v \in W$.\;
				\If{$v \in W$}{
					Add $uv$ to $M_G$.\;
					If $v$ is matched in $M$ with an edge that is now alive then $\phi \gets \phi + 1$\;
					Mark $u$ and $v$ as dead.\;
					\If{there is an edge $uv' \in M$ (i.e. is connected to $u$) where $v'$ is alive}{
						Reveal whether $v' \in W$ and if it is, set $\phi \gets \phi+1$.
					}
				}
			}
		}
	\end{algorithm}
\end{tboxalg2e}

\begin{proof}
	In constructing matching $M_i$ there are two randomizations that are important for the proof of the lemma. The first one is the random permutation $\pi_i$ and the second one is the subsample $S'_i$ of $S_i$.
	
	\smparagraph{The randomization in $\pi_i$.} Fix a 3-augmentable edge $e=\{u,v\} \in S_i$ and suppose that edges $e_v = \{v',v\}$ and $e_u = \{u', u\}$ in $\opt$ are the other two edges in the length 3 augmenting path of $e$. Also consider set $F = E \cap \{ \{v, u'\}, \{u, v'\}\}$. We say that edge $e$ is {\em satisfied} if both edges $e_v$ and $e_u$ are in	 matching $\lfmm{F \cup \{e_v, e_u\}, \pi_i}$ and {\em unsatisfied} otherwise. Intuitively, we would like both endpoints of edge $e$ to be matched in $M_i$ so that they form a length 3 augmenting path. However, if an edge $f \in F$ joins the matching, it kills both $e_u$ and $e_v$ while matching only one endpoint of $e$, which is an undesirable event.
	
	One can confirm that if the lowest-rank edge in $F \cup \{e_u, e_v\}$ is one of $e_u$ or $e_v$, which happens with probability at least $1/2$ since $|F|\leq 2$, then $e$ will be satisfied. Therefore, in expectation, at least half of the edges in $S_i$ will be satisfied.	Furthermore, for the edges in $S_i$, whether one of them is satisfied is completely independent of that of others since the length 3 augmenting paths in $M_0 \oplus \opt$ are vertex disjoit. As a result, by a simple application of Chernoff bound, we get that the number of satisfied edges should w.h.p. be in range $\frac{|S_i|}{2} \pm O(\sqrt{\frac{|S_i|}{2}\log n})$. 
	
	The bound above on the number of satisfied edges is the only property of the randomization in $\pi_i$ that we require for this lemma. That is, the rest of the proof works even if $\pi_i$ is chosen adversarially but satisfies this property. 
	
	
	\smparagraph{The randomization in subsampling $S'_i$.} Consider the bipartite induced subgraph $H=G[V(S_i) \times B_i]$ of $G$. Observe that garph $G_i$ is equivalent to the graph obtained by taking $H$ and removing all of its nodes that are in $V(S_i \setminus S'_i)$. We analyze the following equivalent process of constructing matching $M_i=\lfmm{G_i, \pi_i}$ that gradually reveals subsample $S'_i$ (and thus subgraph $G_i$ of $H$): We initialize $M_i \gets \emptyset$, initially mark each vertex as {\em alive}, and then iterate over the edges of $H$ in the order induced in $\pi_i$. Upon visiting an edge $uv$ with $u \in V(S_i)$ and $v \in B_i$, if either $u$ or $v$ is {\em dead} (i.e., not alive) we discard $uv$. Otherwise, we call $uv$ a {\em potential-match} and then reveal whether $u \in V(S')$ by drawing an $\epsilon$-Bernoulli random variable. If $u \not\in U'$, no edge connected to $u$ can be added to $M$, thus we mark $u$ as dead and discard $uv$. If $u \in U'$, we add $uv$ to $M$ and then mark both $u$ and $v$ as dead as they cannot be matched anymore. One can confirm that in the end of this process, $M$ is precisely equivalent to matching $\lfmm{G[U' \cup V], \pi}$.
\end{proof}


\begin{claim}
%	\label{cl:layerwithlargesize}
	There exists an integer $j \in [1/\epsilon]$ such that $|L_j| \geq \frac{1}{3} \times \frac{1}{100^{1/\epsilon - j}} |M_0|.$
\end{claim}
\begin{proof}
	Suppose for the sake of contradiction that this does not hold for any $j \in [1/\epsilon]$; then:
	$$
	\sum_{i=1}^{1/\epsilon} |L_i| \leq \sum_{i=1}^{1/\epsilon} \frac{1}{3}\times \frac{1}{100^{1/\epsilon - j}} |M_0| =  \frac{|M_0|}{3 \times 100^{1/\epsilon}} \sum_{i=1}^{1/\epsilon} 100^j < \frac{|M_0|}{3 \times 100^{1/\epsilon}} \times 2 \times 100^{1/\epsilon} < |M_0|.
	$$
	Observe that sets $L_1, \ldots, L_{1/\epsilon}$ partition the edges in $M_0$ and thus it should hold that $\sum_{i=1}^{1/\epsilon} |L_i| = |M_0|$; implying that the equation above is indeed a contradiction.
\end{proof}


In what follows, we assume $i^\star$ is the smallest integer that satisfies the condition of Claim~\ref{cl:layerwithlargesize}.


\begin{lemma}
%	\label{lem:augmentamountperlayer}
	There is an absolute constant $\delta > 0$ such that w.h.p.,
	$$
	\mu(M_0 \cup M_{i^\star}) \geq \frac{1}{2}\mu(G) + \delta|L_{i^\star}|.
	$$ 
\end{lemma}

\begin{proof}
	We assume that $|M_0| < \frac{1}{2}\mu(G) + \delta|L_i| = (\frac{1}{2} + \frac{\delta|L_i|}{\mu(G)})\mu(G)$ as otherwise matching $M_0$ itself is large enough to satisfy the lemma's statement. By Observation~\ref{obs:length3augpaths}, this means that at least $(\frac{1}{2} - 3\frac{\delta|L_i|}{\mu(G)})\mu(G)$ edges of $M_0$ are 3-augmentable; meaning that the number of edges in $M_0$ that are not 3-augmentable is at most
	$$
	|M_0| - \left(\frac{1}{2} - 3\frac{\delta|L_i|}{\mu(G)}\right) \mu(G) < \left(\frac{1}{2} + \frac{\delta|L_i|}{\mu(G)}\right)\mu(G) - \left(\frac{1}{2} - 3\frac{\delta|L_i|}{\mu(G)}\right) \mu(G) = 4\delta|L_i|.
	$$
	\sbcomment{This means that at least $(1-4\delta)L_i$ edges in $L_i$ are 3-augmentable and by random sampling its edges, we should be able to find $\delta$ fraction of them given that $\delta$ is a small enough constant.}
	
	\sbcomment{Important: Note that some of the found length 3 augmenting paths may be to edges already in $M_0$, but those will be in the previous layers whose size is small.}
\end{proof}

\begin{lemma}
	The matching $M$ returned by Algorithm~\ref{alg:meta} w.h.p. satisfies $|M| \geq (\frac{1}{2} + \frac{1}{2^{O(1/\epsilon)}})\mu(G)$.
\end{lemma}
\begin{proof}
	Observe that $|M| = \mu(M_0 \cup M_1 \cup \ldots \cup M_{1/\epsilon}) \geq \mu(M_0 \cup M_{i^\star})$. Also by Lemma~\ref{lem:augmentamountperlayer}, it holds that $\mu(M_0 \cup M_{i^\star}) \geq \frac{1}{2}\mu(G) + \delta |L_{i^\star}|$ for an absolute constant $\delta > 0$, implying that $|M| \geq \frac{1}{2}\mu(G) + \delta |L_{i^\star}|$. Furthermore, by Claim~\ref{cl:layerwithlargesize}, $|L_{i^\star}| \geq \frac{1}{3 \times 100^{1/\epsilon - i^\star}}|M_0|$. Putting these together, we get that
	$$
	|M| \geq \frac{1}{2} \mu(G) + \delta \left(\frac{1}{3 \times 100^{1/\epsilon - i^\star}}|M_0|\right) \geq \left( \frac{1}{2} + \delta \frac{1}{3 \times 100^{1/\epsilon}} \right) \mu(G) = \left( \frac{1}{2} + \frac{1}{2^{O(1/\epsilon)}} \right) \mu(G),
	$$
	where the third equation follows from $|M_0| \geq \frac{1}{2}\mu(G)$ since $M_0$ is a maximal matching of $G$.
\end{proof}


\begin{lemma}[\cite{DBLP:conf/approx/KonradMM12}]
	Let $G(U, V, E)$ be a bipartite graph and let $\pi$ be an arbitrary permutation over $E$. For any parameter $p \in (0, 1)$, let $U'$ be a subsample of $U$ including each vertex independently with probability $p$; then $$\E\big[|\lfmm{G[U' \cup V], \pi}|\big] \geq \frac{p}{1+p} \mu(G).$$
\end{lemma}



\begin{proof}
	Consider the following equivalent process of constructing $\lfmm{G[U' \cup V], \pi}$ that gradually reveals the subsample $U'$: We initialize matching $M \gets \emptyset$, initially mark each vertex as {\em alive}, and then iterate over the edges in $E$ in the order of $\pi$. Upon visiting an edge $uv$ with $u \in U$ and $v \in V$, if either $u$ or $v$ is {\em dead} (i.e., not alive) we discard $uv$. Otherwise, we call $uv$ a {\em potential-match} and then reveal whether $u$ belongs to $U'$ by drawing an $\epsilon$-Bernoulli random variable. If $u \not\in U'$, no edge connected to $u$ can be added to $M$, thus we mark $u$ as dead and discard $uv$. If $u \in U'$, we add $uv$ to $M$ and then mark both $u$ and $v$ as dead as they cannot be matched anymore. One can confirm that in the end of this process, $M$ is precisely equivalent to matching $\lfmm{G[U' \cup V], \pi}$.
	
	Let us fix a tape of $|U|$ independent $\epsilon$-Bernoulli random variables $\vec{x} = (x_1, x_2, x_3, \ldots, x_{|U|})$ and use it in the following way: Once we encounter the $i$'th potential-match edge $uv$ in the process, we use the value of $x_i$ as the indicator of the event $u \in U'$. Observe that an edge $uv$ joins $M$ if and only if it is a potential-match edge and that $u \in U'$; therefore, if by the end of the process we encounter $k$ potential-match edges, then we have $|M| = \sum_{i=1}^k x_i$. Note that the number of potential-matches, $k$, that we encounter throughout the process is not fixed a priori and depends on the random variables in the tape. Let us further use $k(\vec{x})$ to emphasize on this, i.e., $k(\vec{x})$ denotes the number of potential-math edges encountered for tape $\vec{x}$. Observe that random variable $k(\vec{x})$ is a stopping time for $\vec{x}$. That is, for any integer $i$, we can determine whether $k(\vec{x}) > i$ by only revealing random variables $x_1, \ldots, x_i$. Therefore, we have
	$$
	\E[|M|] = \E\left[\sum_{i=1}^{k(\vec{x})}x_i\right] \stackrel{\text{Wald's equation}}{=} \E[k(\vec{x})] \E[x_1] = \epsilon \E[k(\vec{x})].
	$$
	Next, we prove that $\E[k(\vec{x})]=(1-\epsilon)\mu(G)$. Fix a maximum matching $M_G$ of $G$ and an edge $uv$ in it with $u \in U$. If we see no potential-match edge for $u$ throughout the process above, then $u$ will remain alive. This means that at the time of visiting edge $uv$ in the process, $uv$ has to be a potential-match edge unless $v$ is dead. Recall that $v$ only dies when it is matched to some other vertex $u' \in U'$. Having this, we charge vertex $u'$ for this edge $uv$. Observe that each vertex in $U'$ is charged at most once. Therefore, the total number of $U$ vertices in $M_G$ that do not have a potential-match edge is at most $|U'|$. Since $k(\vec{x})$ denotes the number of potential-match edges, we get that \sbcomment{to be continued...}
	%	$$
	%	k(\vec{x}) \geq \mu(G) - |U'| \qquad \text{thus,} \qquad \E[k(\vec{x})] \geq \mu(G) - \E[|U'|] = 
	%	$$
\end{proof}



\smparagraph{Intuition behind Lemma~\ref{lem:greedyMM}.} As mentioned before, the main idea behind Lemma~\ref{lem:greedyMM} and generally most efficient randomized algorithms for maximal matching is to {\em hide} the edges of the matching from the oblivious adversary through the use of randomization. The result of \cite{misfocs} shows that this can be done by simulating the random greedy maximal matching algorithm. Here, we overview the intuitions behind why this is the case.

Let us fix an edge update and calculate its expected update-time. Suppose that an edge $e$ is being removed; the case of edge insertion is handled similarly. Observe that since the algorithm greedily handles edges in the increasing order of their ranks, removal of $e$ does not affect the matching constructed on the edges with rank in $[0, \pi(e))$. Moreover, Lemma~\ref{lem:sparsification} tells us that the remaining graph after processing the prefix of edges with rank smaller than $\pi(e)$ has maximum degree $d = \min\{\Delta, \widetilde{O}(1/\pi(e))\}$. Therefore once $e$ is removed, we can in time $\widetilde{O}(d)$ go through its relevant neighbors (i.e., those whose eliminator's rank is larger than $\pi(e)$) and see which one of them, if any, should now join the matching. Note that to be able to explore these incident edges in time $\widetilde{O}(d)$, it is crucial that on each endpoint $v$ of $e$, we maintain adjacency list $N(v)$ which is indexed by the edges' eliminator-ranks. 

Another technicality is that because the greedy maximal matching is being maintained here, a single edge update may affect edges beyond its direct neighborhood. The changes form a path or a cycle whose edges alternatively leave and join the matching. But, fortunately, it is known that these paths/cycles are w.h.p. of size at most $O(\log n)$ if the ranking is random, leading only to a multiplicative $O(\log n)$ factor increase to the update-time. Therefore, overall, the update-time is $O(\log n) \times \widetilde{O}(d) = \widetilde{O}(\min\{\Delta, 1/\pi(e)\})$. The dominant term here is $1/\pi(e)$: As the rank drawn on the first edge $e$ being updated gets smaller, we will need to spend more time updating the matching. For instance if $\pi(e) < 1/\Delta$, the update-time will be as large as  $\widetilde{O}(\Delta)$. However, this is not an issue since the rank $\pi(e)$ of edge $e$ is drawn uniformly at random from $[0, 1]$. Therefore we have $\E_{\pi(e)}[\min\{\Delta, 1/\pi(e)\}] = O(\log \Delta)$ and thus the expected update-time is also polylogarithmic.

